Optimal design of calibration signals in space borne gravitational wave detectors

Future space borne gravitational wave detectors will require a precise definition of calibration signals to ensure the achievement of their design sensitivity. The careful design of the test signals plays a key role in the correct understanding and characterisation of these instruments. In that sense, methods achieving optimal experiment designs must be considered as complementary to the parameter estimation methods being used to determine the parameters describing the system. The relevance of experiment design is particularly significant for the LISA Pathfinder mission, which will spend most of its operation time performing experiments to characterise key technologies for future space borne gravitational wave observatories. Here we propose a framework to derive the optimal signals ---in terms of minimum parameter uncertainty--- to be injected to these instruments during its calibration phase. We compare our results with an alternative numerical algorithm which achieves an optimal input signal by iteratively improving an initial guess. We show agreement of both approaches when applied to the LISA Pathfinder case.

==> include/LTP1D_fisher.tex <==
\section{Application to LISA Pathfinder dynamics}

During operations, LISA Pathfinder will run an exhaustive characterisation campaign 
with the objective of calibrating the instrument and to identify the main noise contributions.
Here we consider one these series of experiments which is the calibration 
of the dynamical parameters, i.e. those ones containing the information of the 
join motion of the test masses and the satellite. 
For these particular set of experiments, the calibration will consists in the injection of a 
sequence of sinusoids at different frequencies --- richer signals are not allowed by hardware ---
in some input ports which allow the characterisation of the closed loop parameters. 
Although the LTP allow many different injection ports,
we will consider in the following injection in the two main interferometer 
channels: the drag-free interferometer channel and the differential interferometer channel
which we have previously described as $o_{1,i}$ and $o_{\Delta,i}$, respectively.
For these particular inputs we study three different cases: injection in the $o_{1,i}$,
injection in $o_{\Delta,i}$ and a simultaneous injection in both $o_{1,i}$ and $o_{\Delta,i}$.
The methodology we use can be easily translated to the other situations.

%We will therefore 
%study this system as 4 independent experiments,
%\begin{equation}
%{\bf F} =  {\bf F^{(11)}} + {\bf F_{\omega_\Delta}^{(21)}} + {\bf F_{\delta_{21}}^{(21)}} + {\bf F^{(22)}}
%\end{equation}
%where each of these is a N$\times$N matrix, where N is the number of parameters. For instance, the elements ${\bf F^{(11)}}$ would be:
%\begin{equation}
%{\bf F^{11}} =
%\left(
%\begin{array}{ccccc}
%F^{(11)}_{G_{\rm df},G_{\rm df}} & F^{(11)}_{G_{\rm df},\omega^2_1} & \ldots & \ldots & F^{(11)}_{G_{\rm df},\delta_{21}} \\
%						 	& & & & \\
%			\vdots		& & \ddots & & \vdots \\
%							& & & & \\
%F^{(11)}_{\delta_{21},G_{\rm df}} 			&  & 		\ldots	& \ldots &  F^{(11)}_{\delta_{21},\delta_{21}} 
%\end{array}
%\right) 
%\end{equation}
%where, for instance
%\begin{equation}
%F^{(11)}_{G_{\rm df},G_{\rm df}}= \lbrace {\bf \Sigma}^{-1} \rbrace_{11} 
%\left[ \partial_{G_{\rm df}} H^{11}(\Theta) \right]^T  \left[ \partial_{G_{\rm df}} H^{11}(\theta)  \right]
%\end{equation}

\subsection{Injection in the differential channel: contribution~$F_{m2p2,ij}$ }
We start the analysis with the simplest case. Given the simplified version 
of the LTP that we use in our analysis, when an injection is applied to the second
channel it will only it will imply that the measured signal appears only in this
same channel, since we assume the cross-coupling $H_{12}$ to be zero.
The  contribution to the Fisher matrix due to 
such an input can be expanded in four terms:
\begin{eqnarray} 
 F_{ij}   & = & \sum_{m,p} F_{m2p2,ij}  \nonumber \\
 & = & F_{1212,ij} + F_{1222,ij} + F_{2212,ij} + F_{2222,ij} \label{eq.F2222}
\end{eqnarray}

where the indices $i$ and $j$ run over the parameters.
From these terms, only the last one $F_{2222,ij}$ is different
from zero since the rest contain the transfer function $H_{12}$.
Eq.\ref{eq.termDef} becomes
\begin{eqnarray}
F_{2222,ij}  & = &   \lbrace {\bf \Sigma}^{-1} \rbrace_{22} \times \nonumber \\
& & \left[ \partial_{\theta_i} H_{22}(\omega) \right]^T 
\left[  \partial_{\theta_j} H_{22}(\omega) \right]
\,| o_{i\Delta} |^2
\label{eq.F2222}
\end{eqnarray}

Due to this simplification, we will be able to describe this problem 
in analytical terms. The unique transfer function involved is $H_{22}$ 
---Eq.~(\ref{eq.H22})--- which depends on two parameters, 
$G_{\rm lfs}$ and $\omega_2$. 
The covariance term $ {\bf \Sigma}^{-1} \rbrace_{22} $ 
can be found in Appendix \ref{sec.AppNoise}
Eq.(\ref{eq.F2222}) turns into a $2\times 2$  
matrix that we can easily decompose in the related eigenvectors,
\begin{equation}
\vec{u_1} = 
\left[ 
\begin{array}{c}
-\frac{G_{\rm lfs}}{\omega^2-\omega_2^2} \\
1 \\
\end{array} \right]
\quad
\vec{u_2} = 
\left[ 
\begin{array}{c}
\frac{\omega^2-\omega_2^2}{G_{\rm lfs}} \\
1
\end{array}
\right]
\end{equation}
and associated eigenvalues,
\begin{eqnarray}
\lambda_1 & = & 0 \nonumber \\
\lambda_2 & = &  \lbrace {\bf \Sigma}^{-1} \rbrace_{22} \times \nonumber \\
 &   &  \frac{H_{\rm lfs}^2 \left(G_{\rm lfs}^2+\left(\omega ^2-\omega^2_2\right)^2\right)}
{\left(G_{\rm lfs}^2 H_{\rm lfs}^2+\left(\omega ^2-\omega^2_1\right)^2+
2 G_{\rm lfs}\, Re\left[H_{\rm lfs} \right]\left(-\omega ^2+\omega^2_2\right)\right)^2} \nonumber \\ 
\end{eqnarray}
There is only one direction with a related non-zero eigenvalue, $\lambda_2$. 
Since eigenvalues are directly related to the inverse 
of the expected uncertainty on the associated parameter, 
we conclude that the direction $\vec{u}_1$ has an associated uncertainty 
that tends to infinity.

It is important to notice at this point that the analysis we perform in the frequency 
domain implicitly assumes a unique frequency, i.e. 
an input signal which is a sinusoid at a given frequency. 
In the following section we explore which information
can we obtain in such a case. Later, we expand the analysis
to a sequence of sinusoids with different frequencies.

\subsubsection{Single tone input: undetermined solution \label{sec:inj2_1sin}}
If we assume that the content of our input signal is a sinusoid with a fixed frequency, 
we know from the previous eigendecomposition that we will not be able to 
solve the problem since we have only one valid eigenvector for a 2-dimensional 
problem. Nonetheless, we explore the single frequency solution in order
to determine how much information can we get from the system in such a case.

As previously explained, we want to express the directions 
defined by the eigenvectors in 
terms of the original directions, which were given by the original
parameters, i.e. the unit vector $ [\hat G_{\rm lfs},\hat \omega_2]$. 
We thus need to rotate the original basis 
according to the new directions, given by the normalised eigenvectors 
$[\hat u_1,\hat u_2]$, which is achieved by applying the rotation matrix {\bf R} to the original vector
\begin{eqnarray}
\vec{\zeta} &=&  {\bf R} \cdot \vec{v}\\
&=& \left(
\begin{array}{cc}
\hat u_{1,x} & \hat u_{2,x} \\
\hat u_{1,y} & \hat u_{2,y} 
\end{array}
\right)
\cdot 
\left(
\begin{array}{c}
\hat G_{\rm df}\\
\hat \omega_1^2
\end{array}
\right)
\end{eqnarray}
where we labelled $x$ and $y$ the two components of the vector. 
By doing this operation and keeping the only non-zero eigenvalue we obtain the following combination of parameters
\begin{equation}
\zeta = \frac{G_{\rm lfs}}{\sqrt{1+\left[\frac{G_{\rm lfs}}{\omega ^2-\omega^2_2}\right]^2}}+
\frac{\omega^2_2}{\sqrt{1+\left[\frac{\omega ^2-\omega^2_2}{G_{\rm lfs}}\right]^2}}
\end{equation}
 with associated error $(\sigma_2^2 = \lambda_2^{-1})$
\begin{widetext}
\begin{equation}
\sigma_{\zeta}  =  \left[ \lbrace {\bf \Sigma}^{-1} \rbrace_{22} \right]^{-1/2} \times 
\left[ \frac{H_{\rm lfs}^2 \left(G_{\rm lfs}^2+\left(\omega ^2-\omega^2_2\right)^2\right)}
{\left(G_{\rm lfs}^2 H_{\rm lfs}^2+\left(\omega ^2-\omega^2_2\right)^2+
2 G_{\rm lfs}\, Re \left[H_{\rm lfs} \right] \left(-\omega ^2+\omega^2_2\right)\right)^2}  \right]^{-1/2}
\end{equation}
\end{widetext}

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.49\textwidth]{figs/FisMat_LTP_5params_F2222_withNoise} 
\caption{eigevalues lambda2. \label{fig.lambda2}}
\end{center}
\end{figure}

In Fig.~\ref{fig.lambda2} we evaluate the previous expressions for different values of the 
calibration parameter $G_{\rm lfs}$, which turns out to be the one with major impact in the curves.
As seen in the plot, the parameter has a direct impact on the expected error for a given frequency input
not only in terms of the magnitude but it can also shift in frequency the value of the expected maximum.  
To further explore the meaning of these results we can study a natural limit for this expression, which 
is to assume that we inject a sinusoid at a frequency corresponding to the stiffness of the second test mass, i.e. $\omega \rightarrow \omega_2$. This leads the following results
\begin{eqnarray}
\zeta & \rightarrow & \omega^2_2 \nonumber \nonumber \\
\sigma_{\zeta} & \rightarrow & \frac{1}{G_{\rm lfs} H_{\rm lfs}}
\end{eqnarray}
which implies that, by imposing this particular limit, we are able to break the degeneracy of the system
and reach an analytical prediction for the error on the stiffness in this injection scheme. However, this is not necessarily an optimal solution since, as previously explained, we are dealing with a single frequency injection scheme which leads to singular Fisher matrix. In the following section we move to the two frequencies injection, overcoming this constraint.

\subsubsection{Two tones input: full-rank solution \label{sec:inj2_2sin}}

In order to combine the information of more than one sinusoid frequency in the 
input signal we add the Fisher matrices corresponding to each frequency. 
Taking into account, as before, that only one term in equation (\ref{eq.F2222}) 
is different from zero, our experiment will therefore be described by
\begin{equation}
F_{2222,ij} = \sum^{N}_{k} \bar F_{2222,ij}(\omega_k)
\end{equation}
where each $\bar F_{2222,ij}(\omega_k)$ corresponds to the contribution 
of a single sinusoid injection to the final experiment's Fisher matrix. 
We explore the case $N=2$, i.e. an input signal composed by two sinusoid
since the experiment being analysed implies only the term $F_{2222}$ and 
therefore only derivatives of the transfer function $H_{22}$ are being computed 
in the Fisher matrix. Hence, only two parameters enter the analysis: $\rm G_{\rm lfs}$ and $\omega^2_2$. 
\begin{figure*}[t]
\begin{center}
\includegraphics[width=0.42\textwidth]{figs/FisMat_LTP_2params_H21_2sinInjection_withNoise_w1_w2.png} 
\includegraphics[width=0.42\textwidth]{figs/FisMat_LTP_2params_H21_2sinInjection_withNoise_w1_w2x50.png} 
\includegraphics[width=0.42\textwidth]{figs/FisMat_LTP_2params_H21_2sinInjection_withNoise_w1x50_w2.png}
\includegraphics[width=0.42\textwidth]{figs/FisMat_LTP_2params_H21_2sinInjection_withNoise_w1x50_w2x50.png} 
\caption{\emph{Top:} Determinant of the $F_{2222}$ contribution for a standard configuration of the
instrument with $G_{df} = 1$,  $G_{sus} = 1 $ ,$\omega^2_1 = -11 \times 10^{-6}$, 
$\omega^2_1 = -22 \times 10^{-6}$./ \emph{Bottom:} The determinant of $F_{2222}$ when we set
  $G_{sus} = 0.5 $. \label{fig.F2222det} }
\end{center}
\end{figure*} 



We first explore the rank of the $F_{2222,ij}$ matrix when evaluated for different
combinations of these two input frequencies. Given that $F_{2222,ij}$ depends on two parameters,
results show that most combinations of frequencies are able to reach the condition 
$\rm rank(F_{2222,ij}) \ne 2$. In fact only when the two frequencies are equal --and we come back 
to our previous case-- we will not be in a full-rank situation.
This allows us to go one step further and explore which combination of frequencies
are optimal, in the sense of maximising the Fisher matrix, i.e. minimising the ellipsoid 
error volume in the parameters space.  
In Fig.~\ref{fig.F2222det} we explore the determinant using standard numerical values for the 
configuration of the experiment. As expected, the surface shows symmetry since the frequencies can be interchanged 
producing the same output. 
The determinant drops to zero at the diagonal since, as commented above, an injection with
two equal frequencies sinusoid does not lead to a full rank solution.

In this particular configuration the maximum is found for the input frequencies 
$\rm f_1 = 1.2$\,mHz and $\rm f_2 = 0.91$\,mHz. With this values we can proceed 
to estimate the expected errors on the parameters. As in the single frequency case, 
we need rotate the basis accordingly to the eigenvectors. However, in the current case, 
we can solve the problem numerically for the two frequencies just derived
\begin{eqnarray}
\vec{\zeta} &=&  {\bf R}(G_{\rm sus} ,\omega^2_2;\omega_1 , \omega_2 ) \cdot \vec{v} \nonumber \\
&=& \left(
\begin{array}{cc}
-0.999 & 0.0001\\
0.0001 & 1 
\end{array}
\right)
\cdot 
\left(
\begin{array}{c}
\hat G_{\rm df}\\
\hat \omega_1^2
\end{array}
\right)
\end{eqnarray}                         
where we notice that the selected optimal frequencies are able to disentangle the two parameters up to 
a factor $1\times 10^{-4}$. The inverse of the eigenvalues tells us about the associated error to each 
of the directions of these eigenvectors.
\begin{eqnarray}
\sigma^2_{\xi_1} & = &  0.3  \nonumber\\
\sigma^2_{\xi_2} & = & 3 \times 10^{-9} \nonumber
\end{eqnarray}
If we neglect the cross terms, we find an estimate of the expected error for the two 
parameters  intervening in the experiment when a signal is injected in the differential channel
\begin{eqnarray}
\sigma_{G_{\rm sus}} & = & \sqrt{\sigma^2_{\xi_1} + \sigma^2_{\xi_1,\xi_2}}    \simeq \sigma_{\xi_1}  = 0.3 \nonumber\\
\sigma_{G_{\omega^2_2}} & = & \sqrt{\sigma^2_{\xi_2} + \sigma^2_{\xi_2,\xi_1}}   \simeq \sigma_{\xi_2} =  3 \times 10^{-9} \nonumber
\end{eqnarray}

\subsubsection{Comparing analytical results against numerical input design}

With the previous analysis we are now in a condition to compare the results obtained analytically 
with the prediction of the numerical algorithm based on the dispersion function -- Eq.~\ref{eq.dispersion}.
To do so, we repeat the same approach previously implemented for the harmonic oscillator, i.e. injecting
a white noise input to the input channel being currently analysed. In this particular case, 
we consider as a initial our initial input a white noise time series of 18\,000\,s and 
$\rm \sigma = 10^{-5}\,m^2$ applied in the differential channel of the LPF.

In the upper panel of Fig.~\ref{fig.F2222compare} we show the evolution of the power spectrum 
of the input signal as retrieved by different iterations of the numerical optimisation algorithm.
The algorithm promotes one frequency at $\rm f = 1.2$\,mHz. To compare this result with
the analytical approach we have previously derived in section \ref{sec:inj2_2sin}, 
we plot in the lower panel of Fig.~\ref{fig.F2222compare} the value of the determinant of 
$F_{2222,ij}$ when injecting two sinusoids. In order to ease the comparison we fix the frequency
of one input sinusoid and plot the determinant value in terms of the frequency of the second injected
signal. This is equivalent as to represent slices of the lower panel of Fig.~\ref{fig.F2222det}.
When doing that we observe that the maximum of the determinant 
stays at the same frequency ---the same as the numerical algorithm retrieves, $\rm f = 1.2$\,mHz --- 
for whatever other input frequency we select. There is however a change in the global maximum of
the determinant depending on which are the two input frequencies selected, which indicates that although
the peak frequency $\rm f = 1.2$\,mHz is a good injection choice, the combination with a second 
frequency  ---$\rm f = 0.91$\,mHz for the chosen parameters --- would lead to an optimal injection 
in terms of the expected error on the parameters. An important feature to notice as well when evaluating the
determinant is the notch appearing for each curve. These would represent the situation where the two frequencies
of the injected sinusoid would be equal. As shown in section~\ref{sec:inj2_1sin}, a single sinusoid 
injection yields a Fisher matrix with rank~=~1 which explains the sudden drop of the determinant 
since the determinant of a non-full-rank determinant is exactly zero. This is observed as well in the 
\emph{valley} on the diagonal of both panels in Fig.~\ref{fig.F2222det}.

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.49\textwidth]{figs/optSignal_numAnalysis_ssm_injch2_input} 
\includegraphics[width=0.49\textwidth]{figs/optSignal_numAnalysis_ssm_injch2_det} 
\caption{...\label{fig.F2222compare}}
\end{center}
\end{figure} 

%\subsection{Injection in the drag-free channel: contribution~$F_{m1p1,ij}$ }
%In the next level of complexity we consider an injection in the drag-free channel.
%Opposite to the previous case, the non-zero cross-coupling term $S_{21}$
%will produce a response in the in the differential channel which, 
%in terms of the present analysis, imply that more parameters can be extracted from the 
%analysis. 
%This can be easily seen from the terms contained in the Fisher matrix for this
%particular injections:
%\begin{eqnarray} 
% F_{ij}   & = & \sum_{m,p} F_{m1p1,ij}  \nonumber \\
% & = & F_{1111,ij} + F_{1121,ij} + F_{2111,ij} + F_{2121,ij} \label{eq.Fm1p1}
%\end{eqnarray}
%
%where again the indices $i$ and $j$ run over the parameters.
%In this case, the transfer functions being evaluated in 
%these terms are $H_{11}$ and $H_{21}$, both of them 
%different from zero and dependent on the parameters
% $\lbrace G_{\rm df}, G_{\rm lfs}, \omega_1, \omega_2, S_{21} \rbrace$,
%which define the subset that we will be able to estimate with an 
%experiment that injects a sequence of sinusoids in the drag-free 
%control loop channel.
%
%

% \subsection{Simultaneous injection in both channels }



%
%\subsection{Injection on first channel with matched stiffness}


% 
%\begin{table}[h]
%\begin{center}
%\begin{tabular}{|c|c|}
%\hline
%{\bf New parameter $\lim_{\omega \rightarrow \omega^2_1} \zeta$} & 
%{ \bf Error on parameter ($\lim_{\omega \rightarrow \omega^2_1}  \sigma_{\zeta}$)} \\
%\hline
%   & \\
%$\omega^2_1$ &   
%$\frac{1}{G_{\rm df}^2 H_{\rm df}^2}$\\
%   & \\
%\hline
%\end{tabular}
%\end{center}
%\end{table}


%\subsection{Numerical analysis}
%
%In the following we evaluate the previous equations for a LTP with fixed parameters. 
%The system is defined by the following parameters: $\lbrace {\rm G_{df}}=1, \omega^2_1 = -11 \times 10^{-7}, {\rm G_{lfs}} = 1, \omega^2_2~=~-22~\times~10^{-7}, \newline \delta_{21}~=~1~\times 10^{-4} \rbrace$
%Results evaluated in the frequency band are shown in Fig. \ref{fig.AllHs}.
%Although we split the problem in the four contributions coming from the four transfer functions, the minimum variance is found to be for two frequencies: $\rm f = 0.15\, Hz$ and $\rm f = 0.2\, mHz$. This is due to the that the minimum of the transfer functions coincides for $H^{11}$ and  $H^{21}_{\delta21}$, the minimum is the same for $H^{22}$ and  $H^{21}_{\omega_\Delta}$ as well.
%
%\begin{figure}[t]
%\begin{center}
%\includegraphics[width=0.49\textwidth]{figs/FisMat_LTP_5params_All} 
%\caption{Expected variance for the $\zeta$ parameter for each transfer function. The variance 
%corresponds to an sinusoidal input at the given frequency. \label{fig.AllHs}}
%\end{center}
%\end{figure}
%
%In order to design a meaningful experiment we need to combine all contributions to evaluate the Fisher matrix. Our framework allows now to reconstruct different experiments by combining the different contributions of the Fisher matrix. 
%For our particular model, to compute the overall Fisher matrix for an injection signal applied to the first channel we will need to add $\bf F^{(11)}$, $\bf F^{(21)}$ and $\bf F^{(21)}$, Instead, a signal injected to the differential channel only contributes with $\bf F^{(22)}$. We consider as well experiments where signals are injected to both channels at the same time, which naturally means to combine all Fisher matrix contributions.
%
%
%In table \ref{tbl.Exps} we compute the rank of the Fisher matrix for different combinations of applied signals for the different channels and for the two frequencies that we have previously seen that maximise the eigenvalues. We also consider experiments with matched stiffness, i.e. experiments where we artificially set $\omega^2_1 = \omega^2_2$
%
%The maximum rank achieved is 4 for the case of a simultaneous injection in both channels at 
%an injection frequency $\rm f =0 .15 \, Hz$, both for standard and matched stiffness case. 
%Since the model is 5 parameters, we conclude that there is no single experiment in the current list which can be used to fully determine our system. 
%However, as shown in last entries of the table, a combination of two single sinusoid experiments would be enough to determine all parameters. It is important to notice that this is not fulfilled for any frequencies and that it requires that one of this two experiments must be in the situation of matched stiffness.
 
%\begin{table*}[t]
%\begin{center}
%\begin{ruledtabular}
%\begin{tabular}{l|c|c|c}
%{\bf Experiment } & {\bf Injection }  &  \bf Injection  & \bf Fisher matrix  \\ 
%{\bf  name} & {\bf  channel}  &  \bf frequency [mHz] & \bf rank \\ 
%\hline
%\multicolumn{4}{c}{\sl Standard Experiments} \\
%\hline
%Injx1($\omega_1$) & $x_1$  								& 	150		& 3 \\
%Injx12($\omega_1$)   & $x_{12}$ 						&  150		& 1 \\
%InjBoth($\omega_1$)  &    $x_1$ \& $x_{12}$  	& 	150		& 4  \\
%\cline{2-4}
%Injx1($\omega_2$) &  $x_1$  								& 2   & 2 \\
%Injx12($\omega_2$)   &  $x_{12}$  						& 2  & 1 \\
%InjBoth($\omega_2$)  &  $x_1$ \& $x_{12}$  		& 2   &  2 \\
%\cline{2-4}
%InjBoth($\omega_1,\omega_2$)  &   $x_1$ \& $x_{12}$  &  2 \& 150 & 2  \\
%\hline
%\multicolumn{4}{c}{\sl Matched Stiffness Experiments} \\
%\hline
%InjMatx1($\omega_1$) & $x_1$  								& 	150		& 3 \\
%InjMatx12($\omega_1$)   & $x_{12}$ 						&  150		& 1 \\
%InjMatBoth($\omega_1$)  &    $x_1$ \& $x_{12}$  	& 	150		& 4 \\
%\cline{2-4}
%InjMatx1($\omega_2$) &  $x_1$  								& 2   & 1\\
%InjMatx12($\omega_2$)   &  $x_{12}$  						& 2  & 1\\
%InjMatBoth($\omega_2$)  &  $x_1$ \& $x_{12}$  		& 2   &  2 \\
%\cline{2-4}
%InjMatBoth($\omega_1,\omega_2$)  &   $x_1$ \& $x_{12}$  & 2 \& 150 & 1 \\
%\hline
%\multicolumn{4}{c}{\sl Combination of Experiments} \\
%\hline
%Injx1($\omega_2$)  +  InjMatBoth($\omega_1$) & -- & -- & 4 \\
%Injx1($\omega_1$)  +  InjMatBoth($\omega_2$) & -- & -- & 4 \\
%Injx1($\omega_1$)  +  InjMatBoth($\omega_1$) & -- & -- & 5 \\
%\hline
%\end{tabular}
%\end{ruledtabular}
%\end{center}
%\end{table*} 
% 

